Construction of time-varying ISS-Lyapunov Functions for Impulsive Systems

Time-varying ISS-Lyapunov functions for impulsive systems provide a necessary and sufficient condition for ISS. This property makes them a more powerful tool for stability analysis than classical candidate ISS-Lyapunov functions providing only a sufficient ISS condition. Moreover, time-varying ISS-Lyapunov functions cover systems with simultaneous instability in continuous and discrete dynamics for which candidate ISS-Lyapunov functions remain inconclusive. The present paper links these two concepts by suggesting a method of constructing time-varying ISS-Lyapunov functions from candidate ISS-Lyapunov functions, thereby effectively combining the ease of construction of candidate ISS-Lyapunov functions with the guaranteed existence of time-varying ISS-Lyapunov functions.

==> chapters/02b_example_superiority.tex <==
\subsection{Example}
%There exist impulsive systems for which ISS cannot be proved with the approach of candidate ISS-Lyapunov functions (e.g. \cite{Dashkovskiy2013}). An example of such a system can be given as follows: 
We provide an example to illustrate how our ISS-Lyapunov functions apply to impulsive systems with simultaneous instability in both continuous and discrete dynamics.
Consider the two-dimensional system in $\R^2$ equipped with Euclidean norm $\norm{\ph}$ and $u \in \R$,
\begin{align}\label{eq:IDEexample2}
	\begin{aligned}
		\dot{x}(t) &= Ax(t), \qquad &&t \in \R_0^+ \setminus S, \\
		x(t) &= g\!\para{x^-(t),u}, \qquad &&t \in S,
	\end{aligned}
\end{align}
where 
$A := \para{
\begin{smallmatrix}
	1	&1 \\
	-1	&1
\end{smallmatrix}
}$, $g\!\para{\para{
\begin{smallmatrix}
    x_1 \\
    x_2
\end{smallmatrix}
},u} := \para{
\begin{smallmatrix}
	2 x_1 \\
	u \tanh(x_2)
\end{smallmatrix}
}$
with $S = \braces{t_i}_{i \in \N}$, and $t_i = \frac{\pi}{2} i$ for $i \in \N$.

Note that the impulsive system described by \eqref{eq:IDEexample2} is strictly unstable in both components of the flow and the direction of the first unit vector of the jumps. Only the jump direction of the second unit vector is stable. 

%We next prove by contradiction that there does not exist a candidate ISS-Lyapunov function for this system as follows. Let there exist a candidate ISS-Lyapunov function and consider the case with unstable flows and stable jumps. By \cite[Theorem~3]{Dashkovskiy2013}, $\alpha(s) < s$ for all $s < 0$ must be fulfilled, but then $V((2s,0)^T) < V((s,0)^T)$ for all $s \neq 0$ which is a contradiction to Condition (3.1), i.e., there must exist a $\mathcal{K}_\infty$-function $\psi_2$ such that $V(x) < \psi_2(\norm{x})$. Hence, we cannot find a candidate ISS-Lyapunov function for system~\eqref{eq:IDEexample2}. 

It can be shown that
\begin{align}\label{eq:LyapunovfunctionExamp2}
    V(t,x) = e^{-4(t-t_n)} x^T R\!\para{t-t_n}D R^T\!\para{t-t_n}x,
\end{align}
where $n = \max\!\braces{i \in \N\,\middle| \, t_i \leq t}$, 
$R$ is the rotation matrix and $D$ is the diagonal matrix defined by $R(t) = \para{
    \begin{smallmatrix}
        \cos(t)     &\sin(t) \\
        -\sin(t)    & \cos(t)
    \end{smallmatrix}
    }
$ and $D =
\para{
    \begin{smallmatrix}
        \frac{1}{4} &0 \\
        0           &2e^{2 \pi}
    \end{smallmatrix}
    }$,
% \begin{align*}
%     R(t) = 
%     \begin{pmatrix}
%         \cos(t)     &\sin(t) \\
%         -\sin(t)    & \cos(t)
%     \end{pmatrix}
%     ,\quad D =
%     \begin{pmatrix}
%         \frac{1}{4} &0 \\
%         0           &2e^{2 \pi}
%     \end{pmatrix},
% \end{align*}
respectively. Hence, \eqref{eq:LyapunovfunctionExamp2} fulfills all the conditions given in Definition \ref{def:LyapunovFunction} with $\chi(s) = 8 e ^{6 \pi} s^2$, therefore being an ISS-Lyapunov function. By the next theorem, we can conclude that system \eqref{eq:IDEexample2} is indeed ISS.

Note that the ISS result in \cite{Dashkovskiy2013} does not apply to system \eqref{eq:IDEexample2} because both the flow and jumps are simultaneously unstable.


%For more intuitive insights on the differences between candidate ISS-Lyapunov functions and our proposed time-varying ISS-Lyapunov functions, we refer to Remark \ref{rem:differenceLFandCLF}.%cannot show ISS of system \eqref{eq:IDEexample2} as the essential mechanism of this type of theorems (e.g. \cite{Dashkovskiy2013}) is injured. There, stability is achieved by balancing the unstable behavior of the flow and jump respectively with stable behavior of the opposite system component. This approach does not work if the neutralization of this counteracting cannot be split accordingly.
% \begin{enumerate}
%     \item Obviously,
%     \begin{align*}
%         \frac{1}{4}e^{-2\pi} \norm{x}^2 \leq V(t,x) \leq 2 e^{2\pi} \norm{x}^2
%     \end{align*}
%     holds for all $(t,x) \in \R^+_0 \times \R^2$.
%     \item The time-derivative of $V$ along the trajectories of the system \eqref{eq:IDEexample2} is given by
%     \begin{align*}
% 		&\frac{\diff}{\diff t} V(t,x) \\
% 		&= -4 e^{-4(t-t_n)}x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} x \\
% 		&\quad + 2 e^{-4(t-t_n)} x^T R\!\para{t-t_n} D \dot{R}^T\!\para{t-t_n} x \\
% 		&\quad + 2 e^{-4(t-t_n)} x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} A x \\
% 		&= -2 e^{-4(t-t_n)}x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} x \\
% 		&= -2 V(t,x)
% 	\end{align*}
% 	for all $x \in \R^2$ and $t \in I \setminus S$ as the second last line follows from the fact that $R^T A = R^T - \dot{R}^T$. Since $2e^{2\pi}\norm{x}^2\geq V(t,x) \geq \chi\!\para{\norm{u}_\infty} = 8e^{6 \pi} \!\norm{u}_\infty^2$ holds, we obtain
% 	\begin{align*}
% 	    V\!\para{t_i,g(x,u)} &= e^0 g(x,u)^T R(0)DR^T(0)g(x,u) \\
% 	    &= x_1^2 + 2e^{2\pi}u^2\tanh^2(x_2) \\
% 	    &\leq e^{-2\pi} \para{2e^{2\pi}x_1^2 + \frac{1}{4}x_2^2} \\
% 	    &= e^{-4\cdot\frac{\pi}{2}}x^T R\!\para{\frac{\pi}{2}}DR^T\!\para{\frac{\pi}{2}}x \\
% 	    &= V(t_i^-,x)
% 	\end{align*}
% 	for each $i \in \N$ and all $x \in \R^2$.
% 	\item For $V(t,x) < \chi\!\para{\norm{u}_\infty} = 8e^{6 \pi} \norm{u}_\infty^2$, we have
% 	\begin{align*}
% 	    V\!\para{t_i,g(x,u)} &= x_1^2 + 2e^{2\pi} u^2\tanh^2(x_2) \\
% 	    &\leq 2e^{2\pi}\norm{x}^2 \cdot \max\!\braces{1, u^2} \\
% 	    &\leq 64e^{10\pi}\norm{u}_\infty^2 \cdot \max\!\braces{1, \norm{u}_\infty^2},
% 	\end{align*}
% 	as by property (1), $\norm{x}^2 \leq 4 e^{2\pi} V(t,x)$ holds.
% \end{enumerate}
% Therefore, $V$ is indeed an ISS-Lyapunov function. By Theorem \ref{thm:Lyapunov}, system \eqref{eq:IDEexample2} is ISS.

==> chapters/04_proof.tex <==
% !TeX spellcheck = en_US
\begin{pf}
    The proof can be partitioned into two steps. For the first step, we prove that for the set
	\begin{align*}
    	A_1(t) := \braces{x \in X \, \middle| \, V(t,x) < \chi\!\para{\norm{u}_{\infty}}}
	\end{align*}
	and every $x_0 \notin A_1(t_0)$, there exists a $\mathcal{KL}$-function $\beta$ such that the inequality $\norm{x(t;t_0,x_0,u)}_X \leq \beta\!\para{\norm{x_0}_X\!, t - t_0}$ holds true if $x(t_*) \notin A_1(t_*)$ for all $t_* \in [t_0,t]$. In the second part, we show that trajectories, once they have reached the set $A_1$, will stay bounded.
	
	Step 1: We first assume that $x(t) \notin A_1$ such that $\V \geq \chi\!\para{\norm{u}_\infty}$ for all $(t,x,u)$.
    Then, by Definition~\ref{def:LyapunovFunction}, the function $V$ fulfills the following inequalities:
	\begin{align}
		\tfrac{\diff}{\diff t} \V  &\leq -\varphi\!\para{\V}, &&t \in I \setminus S, \label{ineq:IDEforV_flow}\\
	\V &\leq \para{\V}^-, &&t \in S. \label{ineq:IDEforV_jump}
	\end{align}
	For brevity, we use $v: I \to \R^+_0,\, v(t) := V\!\para{t,x(t)}$ and denote $v_i := v(t_i)$ and $v^-_i := v^-(t_i)$.
	If the right-hand side of  \eqref{ineq:IDEforV_flow} is non-zero, we can transform \eqref{ineq:IDEforV_flow} to
	\begin{align}\label{ineq:transformIDEforV_flow}
		\frac{\frac{\diff}{\diff t}v}{\varphi(v)}
		\leq\frac{-\varphi(v)}{\varphi(v)} = -1.
	\end{align}
	We explicitly exclude the case $\varphi\!\para{v(t)} = 0$, i.e., $v(t) = 0$ from this inequality. Note that this case is trivial because the trajectories of  \eqref{ineq:IDEforV_flow}--\eqref{ineq:IDEforV_jump} that become equal to zero at some time $t^*$, will remain there for all times $t \geq t^*$.
	
	Integrating \eqref{ineq:transformIDEforV_flow} over the interval $[t_i,t_*]$, $i \in \N_0$, for some $t_* \in [t_i,t_{i+1})$, we obtain
	\begin{align}\label{ineq:estimateFlowVariableUpperBound}
        \int_{v_i}^{v(t_*)} \frac{1}{\varphi(s)}\ \diff s
		= \int_{t_i}^{t_*} \frac{\frac{\diff}{\diff t} v(t)}{\varphi\!\para{v(t)}}\ \diff t\leq -(t_* - t_i),
	\end{align}
	where $s := v(t)$.
	
	We define the function $F: [0,\infty) \rightarrow \R \cup \{-\infty\}$ as
	\begin{align*}
		F(q) := \int_{1}^{q} \frac{1}{\varphi(s)} \ \diff s.
	\end{align*}
	%{\color{blue}$F$ exists for all $q \in [0,\infty)$ because $\varphi$ is strictly positive. The image of $F$ is an interval in $\R$, which is open to the right because $F$ is strictly increasing. Therefore, }
	$F$ is invertible, and $F^{-1}: \image(F) \rightarrow [0,\infty)$ is increasing.
	
	Substituting $F$ into \eqref{ineq:estimateFlowVariableUpperBound}, we get for the left limit $t_* \nearrow t_{i + 1}$, 
	\begin{align} \label{ineq:estimateFlow}
		F(v^-_{i + 1}) - F(v_i) \leq -(t_{i+1} - t_i).
	\end{align}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% find estimate for average impulsive behavior
	We set $n = n(t) := \max\!\braces{n \in \N\,\middle|\, t_n \leq t}$
	in such a way that $t_n$ is the last jump before $t$.
	By the fact that $\varphi$ is positive together with \eqref{ineq:IDEforV_jump}, the inequality $F(v_i) - F(v^-_i)\leq 0$ holds for all $i \in \N$. Combining this with \eqref{ineq:estimateFlow}, we obtain
	\begin{align}
		&F(v(t)) - F(v_0) \nonumber\\
		& = F(v(t))\! -\! F(v_n) \!+ \!\sum\limits_{k = 1}^n F(v_k) \! - \! F(v^-_k) \! + \!
		F(v^-_k) \! - \! F(v_{k - 1}) \nonumber\\
		&\leq - (t - t_n) -\sum\nolimits_{k = 1}^n \para{t_k - t_{k - 1}}
		= -(t - t_0). \label{ineq:estimateV}
	\end{align}
	This is equivalent to
	\begin{align}\label{ineq:vinF}
		v(t) \leq F^{-1}\!\para{F\!\para{v_0} - (t - t_0)}.
	\end{align}
    This inequality fails for $v(t_*) = 0$ for some $t_* \in I$, i.e., when the term $F\!\para{v_0} - (t - t_0)$ vanishes due to the restrictions on \eqref{ineq:transformIDEforV_flow}. But when $v(t_*) = 0$, the inequality \eqref{ineq:vinF} for any $t > t_*$ is trivial as $v(t) = 0$.  However, to circumvent the issue of finding a strictly monotonous $\mathcal{KL}$-function, we define
	\begin{align*}
	    \tilde{\beta}\!\para{v_0, t - t_0}\!&:= F^{-1}\!\!\left(\!F\!\para{v_0} - \para{F\!\para{v_0} - m}\!\para{\!1-\displaystyle e^{\frac{-(t - t_0)}{F\!\para{v_0} - m}}\!}\right) \\
	    &\geq F^{-1}\!\para{F\!\para{v_0} - (t - t_0)}
	\end{align*}
	for $m > - \infty$, where $m := \inf\{\image(F)\}$. Otherwise, we set 
	\begin{align*}
	    \tilde{\beta}\!\para{v_0, t - t_0} := F^{-1}\!\para{F\!\para{v_0} - (t - t_0)}.
	\end{align*}
	Clearly, $\tilde{\beta}$ is strictly increasing in $v_0$ and decreasing strictly to zero in $t - t_0$. We define $\beta \in \mathcal{KL}$, $\beta(r,s) := \alpha_1^{-1}\!\para{\tilde{\beta}\!\para{\alpha_2(r),s}}$, and obtain for $t \in [t_0, t^*]$,
	\begin{align} \label{ineq:asymptoticStabilityOfTrajectory}
		\norm{x(t;t_0,x_0,u)}_X \leq \beta\!\para{\norm{x_0}_X\!, t - t_0},
	\end{align}
	where $t^* := \inf\!\braces{t \in [t_0,\infty] \, \middle| \, \V < \chi\!\para{\norm{u}_{\infty}}}$. Obviously, in case $t^* = \infty$, $t$ is to be chosen in $[t_0, t^*)$.
	
%	Next, we estimate trajectories starting in $\Omega_{t,d}$. As $\Omega_{t,d}$ is a subset of $\braces{x \in X \,\middle|\, \alpha_1\!\para{\norm{x}_X} \leq \alpha_2(a)}$ the inequality $\norm{x(t)}_X \leq \alpha_1^{-1}\alpha_2(a)$ holds.

	Step 2: Next, we  show that trajectories that are in $A_1(t)$ for some $t \in I$, stay bounded for all times. Therefore, we apply \eqref{def:LyapFuncCondition3} from which we can conclude that all trajectories jumping from $A_1^-(t)$ for some $t = t_i$ are bounded by
	\begin{align*}
		A_2(t) := \braces{x \in X \,\middle| \, V(t,x) \leq \alpha_3\!\para{\norm{u}_\infty}}.
	\end{align*}
	It is not possible that the trajectories leave
	\begin{align*}
		&A_3(t) := \overline{A_1(t) \cup A_2(t)} \\
		&= \braces{x \in X \,\middle| \, V(t,x) \leq \max\!\braces{\alpha_3\!\para{\norm{u}_\infty}\!, \chi\!\para{\norm{u}_{\infty}}}}
	\end{align*}
	neither by jump nor by flow because the boundary of $A_1(t) \cup A_2(t)$ is in the complement of $A_1$. From \eqref{ineq:IDEforV_flow}, it follows that $\frac{\diff}{\diff t}\V < 0$ holds on the boundary, and jump inequality \eqref{ineq:IDEforV_jump} prevents the trajectories from leaving $A_3(t)$. We define $\gamma \in \mathcal{K}_\infty$, $\gamma :=\alpha_1^{-1} \circ \max\!\braces{\alpha_3\!\para{\ph}, \chi\!\para{\ph}}$. Then $\norm{x(t;t_0,x_0,u)}_X \leq \gamma\!\para{\norm{u}_\infty}$
	holds for all $t > t^*$.
	From this equation and \eqref{ineq:asymptoticStabilityOfTrajectory}, we can conclude
	\begin{equation*}
		\norm{x(t;t_0,x_0,u)}_X \leq \beta\para{\norm{x_0}_X\!, t - t_0} + \gamma\!\para{\norm{u}_\infty}.
    \end{equation*}
\end{pf}

==> chapters/05_theorem.tex <==
% !TeX spellcheck = en_US
%\section{Converse ISS-Lyapunov Theorem}\label{sec:inverseLyapunovTheorem}


Now we provide the converse ISS-Lyapunov theorem, i.e., for every impulsive system \eqref{eq:ImpulsiveSystem}, which is ISS, there exists an ISS-Lyapunov function so that the problem of determining ISS of a system reduces to finding an ISS-Lyapunov function.

Until now, we were able to work on a maximal level of generality concerning the right-hand side of  impulsive system \eqref{eq:ImpulsiveSystem}. In what follows, we need more regularity conditions. We require system \eqref{eq:ImpulsiveSystem} to satisfy the following Lipschitz continuity assumptions.


% \begin{remark}
% 	Here, we used, and will also use in what follows, the notion of Lipschitz continuity on bounded sets. For non-compact sets, this is not equivalent to local Lipschitz continuity. Lipschitz continuity on bounded sets includes local Lipschitz continuity as each set can be chosen as a neighborhood of a point in $X$ but not vice versa. This can be proved as follows. Let $L_x$ be the Lipschitz constant, and $U_x$ be  the neighborhood of each $x \in X$. We choose a sequence $(x_i)_{i \in \N}$ such that $\bigcup_{i \in \N} U_{x_i}$ is a cover of the ball with radius one. If $X$ is not compact, there is an open cover of the ball with radius one without a finite subcover. Therefore, the supremum of the Lipschitz constants $\sup_{i \in \N}\braces{L_{x_i}}$ might not exist. 
% \end{remark}

\begin{remark}
	Here, we used, and will also use in what follows, the notion of Lipschitz continuity on bounded sets. Lipschitz continuity on bounded sets implies local Lipschitz continuity and on compact sets the notions are equivalent. For non-compact sets, Lipschitz continuity on bounded sets is not equivalent to local Lipschitz continuity.
\end{remark}


Now we state the converse ISS-Lyapunov theorem.

\begin{theorem}\label{thm:inverseLyapunov}
	Let impulsive system \eqref{eq:ImpulsiveSystem} be ISS and satisfy Assumption 1. Then, there exists an ISS-Lyapunov function for system \eqref{eq:ImpulsiveSystem}.
\end{theorem}

A proof of this theorem can be found in our recent paper \task{[cite archive paper, Theorem 2]}.
%For proving Theorem \ref{thm:inverseLyapunov}, we extend the approach given in \cite{Mironchenko2018b} to impulsive systems. However, this extension is not straightforward as it includes significant modifications that take care of the impulsive nature of system \eqref{eq:ImpulsiveSystem}. 

% The proof of Theorem \ref{thm:inverseLyapunov} includes the steps depicted in Fig. \ref{fig:implicationDiagram}. The proof will proceed via an intermediate state called \emph{weak uniform robust asymptotic stability (WURS)}. First, we show that from ISS of system \eqref{eq:ImpulsiveSystem} follows WURS, and afterward, we establish that WURS includes the existence of a Lyapunov function.

% \begin{figure}[htb]
%     \centering
%     \begin{tikzcd}[column sep=3cm, row sep = 2.0cm] % put row sep = 0.8cm
%         \eqref{eq:ImpulsiveSystem} is ISS 
%         \arrow[r, Leftarrow, "Theorem\,\ref{thm:Lyapunov}"]
%         \arrow[d, Rightarrow, "Lemma\,\ref{lem:WURS}"]
%         & $\exists$ ISS-LF for \eqref{eq:ImpulsiveSystem}
%         \arrow[d, Leftarrow, "Lemma\,\ref{lem:WURStoISS}"] \\ 
%         \eqref{eq:ImpulsiveSystem} is WURS 
%         \arrow[r, Rightarrow, "Theorem\,\ref{thm:existenceOfLyapunovFunction}"] 
%         &$\exists$ LF for \eqref{eq:feedbackImpulsiveSystem}
%     \end{tikzcd}
%     \caption{Diagram illustrating the proof of Theorem~\ref{thm:inverseLyapunov}.}
%     \label{fig:implicationDiagram}
% \end{figure}

% In order to introduce WURS, we define a feedback system related to \eqref{eq:ImpulsiveSystem}. Let there exist a function $\eta: X \to \R^+_0$, which is Lipschitz-continuous on bounded subsets of $X$, and a function $\psi \in \mathcal{K}_\infty$ such that $\eta(x) \geq \psi(\norm{x}_X)$ and
% \begin{align}
% 	&\begin{aligned}\label{eq:feedbackImpulsiveSystem}
% 		\dot{x}(t) &= Ax(t) + f\!\para{t,x(t),d(t)\eta\!\para{x(t)}} \\
% 		&=:  Ax(t) + \overline{f}\!\para{t,x(t),d(t)}, \quad &t \in I\setminus S, \\
% 		x(t) &=g_i\!\para{x^-(t),d(t)\eta\!\para{x^-(t)}} \\
% 		&=: \overline{g}_i\!\para{x^-(t),d(t)}, \quad &\hspace{-2em} t =t_i, \ i \in \N ,
% 	\end{aligned}
% \end{align}
% where $d \in D := \braces{d: I \to U \,\middle|\, \norm{d}_\infty\leq 1}$. We denote trajectories of \eqref{eq:feedbackImpulsiveSystem} with initial condition $x(t_0) = x_0$ by $\overline{x}_d(t; t_0, x_0)$ which we abbreviate by $\overline{x}_d(t)$ if possible.

% Next, we provide several definitions.
% \begin{definition}\label{def:StabilityDefinitions}
% 	System \eqref{eq:feedbackImpulsiveSystem} is called
% 	\begin{enumerate}[(i)]
% 		\item \emph{uniformly globally asymptotically stable (UGAS)} if there exists a $\mathcal{KL}$-function $\beta$ such that for all $d \in D$, the inequality $\norm{\overline{x}_d(t; t_0,x_0}_X \leq \beta\!\para{\norm{x_0}_X\!, t - t_0}$ holds for all $x_0 \in X$ and all $t \geq t_0$;
% 		\item \emph{uniformly globally attractive} if for any $C,\eps > 0$ there is a $\delta = \delta(C,\eps) > 0$ such that for all $d \in D$ the inequality $\norm{\overline{x}_d(t; t_0,x_0)}_X \leq \eps$ holds for all $x_0 \in X$ satisfying $\norm{x_0}_X \leq C$ and all $t \geq t_0 + \delta(C,\eps)$;
% 		\item \emph{uniformly globally stable} if there exists a class $\mathcal{K}_\infty$-function $\alpha$ such that for all $d \in D$, $x_0 \in X$ and $t \geq t_0$ the inequality $\norm{\overline{x}_d(t; t_0,x_0)}_X \leq \alpha\!\para{\norm{x_0}_X}$ holds;
% 		\item \label{def:robustForwardCompleteness}\emph{robustly forward complete} if for all $C > 0$ and $\tau > t_0$
% 		\begin{align*}
% 			K(C,\tau) := \sup\nolimits_{x_0 \in \ball_X(C),\, d \in D,\, t \in [t_0,\tau]} \norm{\overline{x}_d(t;t_0,x_0)}_X
% 		\end{align*}
% 		is finite.
% 	\end{enumerate}
% \end{definition}

% \begin{definition}\label{def:WURS}
% 	System \eqref{eq:ImpulsiveSystem} is called \emph{weakly uniformly robustly asymptotically stable (WURS)}, if there exist a function $\eta: X \to \R^+_0$, which is Lipschitz-continuous on bounded subsets of $X$ and $\psi \in \mathcal{K}_\infty$ such that $\eta(x) \geq \psi(\norm{x}_X)$, and  feedback system \eqref{eq:feedbackImpulsiveSystem} is UGAS for all $d \in D$.
% \end{definition}







==> chapters/06_lemma_WURS.tex <==
% !TeX spellcheck = en_US
Now we establish the first part of the proof of Theorem \ref{thm:inverseLyapunov}.
\begin{lemma}\label{lem:WURS}
	If  impulsive system \eqref{eq:ImpulsiveSystem} is ISS, then it is WURS.
\end{lemma}

\begin{pf}
%	First show: from ISS follows WURS
	From the definition of ISS, it follows that there exist functions $\beta \in \mathcal{KL}$ and $\gamma \in \mathcal{K}_\infty$. We define $\alpha(s) := \beta(s,0)$ for all $s \in \R^+_0$. From inequality \eqref{ineq:ISS}, it follows that $\alpha(s) \geq s$ for all $s \in \R^+_0$, which means that $\alpha \in \mathcal{K}_\infty$.
	
	We define $\sigma \in \mathcal{K}_\infty$ as $\sigma(s) \leq \para{\gamma^{-1}\!\para{\tfrac{1}{4} \alpha^{-1}\!\para{\tfrac{2}{3}\alpha^{-1}\!\para{\tfrac{2}{3} s}}} }$, and choose locally Lipschitz continuous functions $\eta: X \to \R^+_0$ and $\psi  \in \mathcal{K}_\infty$  such that  $\psi\!\para{\norm{x}_X} \leq \eta(x) \leq \sigma\!\para{\norm{x}_X}$.
	
	We show that with this definition of $\eta$, the inequality
	\begin{align}\label{ineq:estimategammau}
		\gamma\!\para{\norm{d(t)\eta\!\para{\overline{x}_d(t}}_U} \leq \tfrac{1}{2} \norm{x_0}_X
	\end{align}
	holds for all $t \geq t_0$. We first compute
	\begin{align*}
		&\gamma\!\para{\norm{d(t) \eta\!\para{\overline{x}_d(t}}_U} 
		\leq \gamma\!\para{\sigma\!\para{\norm{\overline{x}_d(t)}_X}} \\*
		&\leq \tfrac{1}{4} \alpha^{-1}\!\para{\tfrac{2}{3}\alpha^{-1}\!\para{\tfrac{2}{3}\norm{\overline{x}_d(t)}_X}}
		\leq\tfrac{1}{9}\norm{\overline{x}_d(t)}_X
	\end{align*}
	which is valid for every $d \in D$, all $x_0 \in X$, and all $t \in I$. By definition, $\overline{x}_d$ is right-continuous, so for each $t_* \in I$, there exists a $\delta > 0$ such that
	\begin{align}
		\gamma\!\para{\norm{d(t) \eta\!\para{\overline{x}_d(t;t_*, x_*)}}_U}
		&\leq\tfrac{1}{9}\!\norm{\overline{x}_d(t; t_*, x_*)}_X\!
		\leq \tfrac{1}{2}\! \norm{x_*}_X \label{ineq:estimategamma}
	\end{align}
	for all $t \in [t_*,t_* + \delta]$, where the last inequality in \eqref{ineq:estimategamma} follows from continuity. The next step is to fix randomly chosen $d \in D$, $t_0 \in I$, and $x_0 \in X$, and define $\overline{t} = \overline{t} (t_0, x_0, d)$ by
	\begin{align*}
		&\overline{t} = \inf \!\braces{t \geq t_0 \,\middle|\, \gamma\!\para{\norm{d(t) \eta\!\para{\overline{x}_d(t}}_U} > \tfrac{1}{2} \!\norm{x_0}_X}\!.
	\end{align*}
	Obviously,  $\overline{t} \in (t_0, \infty]$. We prove by contradiction that $\overline{t} = \infty$. Thus, let us assume that $\overline{t}$ is not equal to infinity. Then, inequality \eqref{ineq:estimategamma} holds for all $t \in [t_0,\overline{t})$. By substituting inequality \eqref{ineq:estimategamma} into \eqref{ineq:ISS}, we obtain
	\begin{align}
		&\norm{\overline{x}_d(t)}_X 
		\leq \beta\!\para{\norm{x_0}_X\!, t - t_0} + \tfrac{1}{2}\norm{x_0}_X \nonumber\\
		&\leq \beta\!\para{\norm{x_0}_X\!, t - t_0} + \tfrac{1}{2}\alpha\!\para{\norm{x_0}_X}
		\leq \tfrac{3}{2}\alpha\!\para{\norm{x_0}}\!. \label{ineq:estimateTrajectoryByIC}
	\end{align}
	System \eqref{eq:ImpulsiveSystem} is bound to the principle of causality, i.e., it only depends on past states. This means that it exhibits the same behavior on the interval $[t_0,\overline{t}]$ for $u \in U_c$ as for
	\begin{align*}
		\tilde{u} =
		\begin{cases}
			u	&t \in [t_0, \overline{t}),\\
			0	&\text{else}.
		\end{cases}
	\end{align*}
	Therefore, we can transform \eqref{ineq:ISS} into
	\begin{align}
		&\norm{\overline{x}_d(\overline{t};t_*,x_*)}_X 
		\leq \beta\!\para{\norm{x_*}_X, \overline{t} - t_*} \nonumber\\
		&+ \gamma\!\para{\sup\nolimits_{t \in [t_*,\overline{t})}\!\braces{\norm{d(t)\eta\!\para{\overline{x}_d(t;t_*, x_*)}}_U}}\!.\label{ineq:ISSmod}
	\end{align}
	As system \eqref{eq:feedbackImpulsiveSystem} is only right-continuous, we need an estimate for limits from the left, which also considers possible jumps.  This estimate is given by 
	\begin{align}
		&\norm{\overline{x}_d(\overline{t})}_X
		= \lim\nolimits_{t_* \nearrow \overline{t}} \norm{\overline{x}_d(\overline{t};t_*,\overline{x}_d(t_*))}_X \nonumber\\
		&\leq \lim\nolimits_{t_* \nearrow \overline{t}}\beta\!\para{\norm{\overline{x}_d(t_*)}_X, \overline{t} - t_*} \nonumber\\
		&\quad + \gamma\!\para{\sup\nolimits_{t \in [t,\overline{t})}\!\braces{\norm{d(t) \eta\!\para{\overline{x}_d\!\para{t_*}}}_U}} \nonumber\\
		&\leq \alpha\!\para{\norm{\overline{x}^-_d(\overline{t})}_X} + \tfrac{1}{2}\norm{\overline{x}^-_d(\overline{t})}_X 
		\leq \tfrac{3}{2}\alpha\!\para{\norm{\overline{x}^-_d(\overline{t})}_X}\!, \label{ineq:estimatexatjump}
	\end{align}
	which is obtained from the semigroup property $\overline{x}_d(\overline{t}) = \overline{x}_d\!\para{\overline{t};t,\overline{x}_d(t)}$ for all $t \in [t_0,\overline{t}]$  and \eqref{ineq:ISSmod}.
	From \eqref{ineq:estimatexatjump} follows
	\begin{align*}
		&\gamma\!\para{\norm{d(\overline{t})\eta\!\para{\overline{x}_d(\overline{t})}}_U}\leq \gamma\!\para{\sigma\!\para{\tfrac{3}{2}\alpha\!\para{\norm{\overline{x}^-_d(\overline{t})}_X}}} \\
		&\leq \tfrac{1}{4}\alpha^{-1}\!\para{\tfrac{2}{3} \alpha^{-1}\!\para{\tfrac{2}{3}\cdot\tfrac{3}{2}\alpha\!\para{\norm{\overline{x}^-_d(\overline{t})}_X}}} \\
		&\leq \tfrac{1}{4}\alpha^{-1}\!\para{\tfrac{2}{3} \norm{\overline{x}^-_d(\overline{t})}_X}
		\leq \tfrac{1}{4}\norm{x_0}_X,
	\end{align*}
	where we have used the definition of $\sigma$ in the second, and \eqref{ineq:estimateTrajectoryByIC} in the fourth inequality.
	
	As $\overline{x}_d$ is right-continuous, there is a neighborhood to the right of $\overline{t}$ such that $\gamma\!\para{\norm{d(t) \eta\!\para{\overline{x}_d(t}}_U} \leq \tfrac{1}{2} \norm{x_0}_X$. This is a contradiction to the definition of $\overline{t}$ and shows the validity of \eqref{ineq:estimategammau} for all $t \geq t_0$.
	Therefore,
	\begin{align}\label{ineq:estimatexetainbeta}
		\norm{\overline{x}_d(t)}_X \leq \beta\!\para{\norm{x}_X, t - t_0} + \tfrac{1}{2}\norm{x}_X
	\end{align}
	holds for all $x \in X$, all $d \in D$, and all $t \geq t_0$, which gives us uniform global stability of system \eqref{eq:feedbackImpulsiveSystem}.
	
	To show uniform global attractivity, we use the fact that there exists such a $\tau_1 =\tau_1\!\para{\norm{x}_X}$ that ${\beta\!\para{\norm{x}_X\!, t} \leq \tfrac{1}{4} \norm{x}_X}$ for all $t \geq \tau_1$. Substituting this term into \eqref{ineq:estimatexetainbeta} yields $\norm{\overline{x}_d(t)}_X \leq \tfrac{3}{4}\norm{x_0}_X$ for all $x_0 \in X$, $d \in D$, and $t \geq \tau_1$. By using similar arguments, we can find a sequence $(\tau_i)_{i \in \N}$ that only depends on $\norm{x_0}_X$ such that
	\begin{align*}
	    \norm{\overline{x}_d(t)}_X \leq \para{\tfrac{3}{4}}^k\norm{x_0}_X
	\end{align*}
	holds for all $x_0 \in X$, $d \in D$, and $t \geq \tau_k$. This implies uniform global attractivity of system \eqref{eq:feedbackImpulsiveSystem}.
	From \cite[Thm. 2.2]{Karafyllis2011},  it follows that system \eqref{eq:feedbackImpulsiveSystem} is UGAS. Therefore,  impulsive system \eqref{eq:ImpulsiveSystem} is WURS by Definition \ref{def:WURS}.
\end{pf}
















































==> chapters/07_proposition_Lipschitzcontinuity.tex <==
% !TeX spellcheck = en_US
\begin{proposition}\label{prop:Lipschitzcontinuity}
	Let Assumption \ref{A1} hold, and system \eqref{eq:ImpulsiveSystem} be WURS. Then, for any $\eta$ as defined in Definition \ref{def:WURS}, the closed-loop system \eqref{eq:feedbackImpulsiveSystem} has robustly forward complete solutions, which are  Lipschitz continuous with respect to initial values in bounded subsets of $X$ and locally Lipschitz continuous on intervals $t \in [t_i,t_{i + 1})$, $i \in N_0$, where the Lipschitz constant depends on the norm of the initial condition $\norm{x_0}_X$.
\end{proposition}

\begin{pf}%{PROOF OF PROP. \ref{prop:Lipschitzcontinuity}}
	The solutions of system \eqref{eq:ImpulsiveSystem} exist for every $t \geq t_0$. This implies that the solutions of system \eqref{eq:feedbackImpulsiveSystem} also exist for every $t \geq t_0$. Let $\eta$ be the function constructed in Definition \ref{def:WURS}. According to Definition \ref{def:WURS}, system \eqref{eq:feedbackImpulsiveSystem} is UGAS. Therefore, for all $C>0$ and all $\tau > t_0$
	\begin{align*}
		\sup\nolimits_{x_0 \in \ball_X(C),\, d \in D,\, t \in [t_0,\tau]} \norm{\overline{x}_d (t;t_0,x_0)}_X \leq \beta(C,0)
	\end{align*}
	exists, and system \eqref{eq:feedbackImpulsiveSystem} is robustly forward complete.
	
	We apply Lemma \ref{lem:LipschitzcontinuityRHS} from the Appendix  to obtain that $\overline{f}$ and $\overline{g}_i$ are Lipschitz continuous in space on bounded subsets of $X$ and uniformly with respect to $t$ and $d$. Therefore, the preconditions of Lemma \ref{lem:Lipschitzcontinuityflow} in the Appendix are fulfilled, i.e., system \eqref{eq:feedbackImpulsiveSystem} has a solution, which is Lipschitz continuous with respect to the initial values in bounded subsets of $X$. From Lemma \ref{lem:LipschitzContinuityInTime} in the Appendix, it follows that the trajectories are locally Lipschitz continuous on intervals $t \in [t_i,t_{i + 1})$, $i \in N_0$, as claimed in the Proposition.
\end{pf}

We now define a Lyapunov function to establish UGAS of feedback system \eqref{eq:feedbackImpulsiveSystem}. This is not an ISS-Lyapunov function as given in Definition~\ref{def:LyapunovFunction} but it provides global asymptotic stability, uniformly with respect to control.
\begin{definition}\label{def:LyapunovFunctionFeedback}
    Let $V: I \times X \to \R_0^+$ be such that $V \in \Cont\!\para{(I\setminus S)\times X,\R_0^+}$ and $V \in \PC(I \times X,\R_0^+)$ hold. We call  $V$ a \emph{Lyapunov function} for  system \eqref{eq:feedbackImpulsiveSystem}, if it fulfills all of the following conditions:
	\begin{enumerate}[(i)]
		\item There exist functions $\alpha_1, \alpha_2 \in \mathcal{K}_\infty$ such that
		\begin{align*}
			\alpha_1\!\para{\norm{\overline{x}}_X} \leq V(t,\overline{x}) \leq \alpha_2\!\para{\norm{\overline{x}}_X} %\label{ineq:LyapunovDefiniteness}
		\end{align*}
		holds true for all $t \in I$ and all $\overline{x} \in X$. %\label{def:LyapFuncCondition1}
		\item There exists a $\varphi \in \mathcal{P}$ %and a continuous function $\varphi: [0,\infty) \rightarrow \R$ with $\varphi(0) = 0$
		such that for all $u \in U_c$ and all solutions $\overline{x} = \overline{x}(t; t_0,x_0,u)$ of \eqref{eq:ImpulsiveSystem}, the inequalities
		\begin{align*}
			\tfrac{\diff}{\diff t}V(t, \overline{x}) &\leq - \varphi\!\para{V(t,\overline{x})}, \quad &&t \in I \setminus S, %\label{ineq:LyapunovFlow} 
			\\
			V\!\para{t_i, \overline{g}_i\!\para{\overline{x}, u}} &\leq V(t_i^-,\overline{x}), \quad &&t_i \in S, %\label{ineq:LyapunovJump}
		\end{align*}
		holds true.
		Here, $\frac{\diff}{\diff t}V(t, \overline{x}) $ is again the Dini-derivative.
	\end{enumerate}
\end{definition}


With Proposition \ref{prop:Lipschitzcontinuity} at hand, the following converse Lyapunov theorem \cite[Thm. 3.4]{Karafyllis2011} delivers the implication from WURS to the existence of a Lyapunov function as given in Definition \ref{def:LyapunovFunctionFeedback} for system~\eqref{eq:feedbackImpulsiveSystem}.

\begin{theorem}\label{thm:existenceOfLyapunovFunction}
    Let system (1) be WURS, and  its solutions be Lipschitz continuous with respect to initial values in bounded subsets of $X$ and locally Lipschitz continuous on intervals $t \in [t_i,t_{i + 1})$, $i \in N_0$, where the Lipschitz constant depends on the norm of the initial condition $\norm{x_0}_X$. Then, there is a Lyapunov function $V$ for system \eqref{eq:feedbackImpulsiveSystem} as given in Definition \ref{def:LyapunovFunctionFeedback}, which is Lipschitz continuous on bounded balls in space and locally Lipschitz continuous on the intervals $[t_i,t_{i + 1})$, $i \in \N_0$.
\end{theorem}

% A proof of this theorem can be found in \cite[Thm. 3.4]{Karafyllis2011}. We have to keep in mind, that UGAS implies URGAOS and the properties HYP and BIC are fulfilled by our definition of a solution. \task{From the Lipschitz continuity in the initial condition follows (REG2) and by using Lemma \ref{lem:LipschitzContinuityInTime} in the Appendix follows local Lipschitz continuity in time and we can conclude (REG3).}



























==> chapters/08_lemma_ISSfunction.tex <==
% !TeX spellcheck = en_US
From the next lemma, we obtain that the existence of a Lyapunov function for feedback system \eqref{eq:feedbackImpulsiveSystem} implies the existence of an ISS-Lyapunov function for system~\eqref{eq:ImpulsiveSystem}.
\begin{lemma}\label{lem:WURStoISS}
    Let there exist a Lyapunov function $V$ for  system \eqref{eq:feedbackImpulsiveSystem} as given in Definition \ref{def:LyapunovFunctionFeedback}, which is Lipschitz continuous on bounded balls in space and locally Lipschitz continuous on the intervals $[t_i,t_{i + 1})$, $i \in \N_0$.
	Then, there exists an ISS-Lyapunov function of the form given in Defintion \ref{def:LyapunovFunction}, which is Lipschitz continuous on bounded subsets of $X$, and locally Lipschitz continuous on $I \setminus S$ such that it is right continuous and the left limit exists.
\end{lemma}
\begin{pf}
	The definition of the Lyapunov function $V$ in Definition \ref{def:LyapunovFunctionFeedback} immediately implies the inequalities \eqref{ineq:LyapunovFlow}--\eqref{ineq:LyapunovJump}
	hold for all $x \in X$ and $u \in \ball_U(\eta(x))$. As a consequence of Definition \ref{def:WURS}, \eqref{ineq:LyapunovFlow}--\eqref{ineq:LyapunovJump} hold for all $x \in X$ and $u \in \ball_U\!\para{\psi\!\para{\norm{x}_X}}$. As $\psi$ is invertible, we can set $\chi := \alpha_1 \circ \psi^{-1}$. By this, $V$ satisfies  \eqref{ineq:LyapunovFlow}--\eqref{ineq:LyapunovJump} without additional restrictions.
	
	It remains to show that the third property of Definition~\ref{def:LyapunovFunction} is fulfilled. We claim that $g_i(0,0) = 0$ for all $i \in \N$. Let us assume $g_i(0,0) \neq 0$. Then, for the trajectories of system \eqref{eq:feedbackImpulsiveSystem} satisfying $\overline{x}^-(t_i) = 0$, it follows that
	\begin{align*}
		\overline{x}(t_i) &= \overline{g}_i\!\para{\overline{x}^-(t_i), d(t_i)} 
		= g_i\!\para{\overline{x}^-(t_i), d(t_i)\eta\!\para{\overline{x}^-(t_i)}} \\*
		&= g_i(0,0) 
		\neq 0.
	\end{align*}
	This means that $\overline{x} = 0$ is not a fixed point, and system \eqref{eq:feedbackImpulsiveSystem} cannot be UGAS. This is a contradiction. Therefore, the claim $g_i(0,0) \neq 0$ holds true.
	
	Let $V\para{t_i,x} < \chi\!\para{\norm{u}_U}$ hold, it follows from \eqref{ineq:LyapunovDefiniteness} that
	\begin{align} \label{ineq:estimateofxinu}
		\norm{x}_X \leq \para{\alpha_1^{-1} \circ \chi}\!\para{\norm{u}_U} = \kappa\!\para{\norm{u}_U},
	\end{align}
	where we define $\kappa \in \mathcal{K}_\infty$, $\kappa(s) = \para{\alpha_1^{-1} \circ \chi}\!(s)$. For $\norm{x}_X \leq C$ and $\norm{u}_U \leq D$, we have
	\begin{align}
		&\norm{g_i(x,u)}_X
		\leq \norm{g_i(x,u)\! - \!g_i(0,u)}_X\! + \!\norm{g_i(0,u)\! - \!g_i(0,0)}_X \nonumber\\
		&\leq L_{g_i}^1(C,D)\norm{x}_X + L_{g_i}^2(C,D)\norm{u}_U \nonumber\\
		&\leq L_{g_i}^1(C,D)\kappa\!\para{\norm{u}_U}\!+\! L_{g_i}^2(C,D)\!\norm{u}_U = \tilde{\alpha}_3\!\para{\norm{u}_U}\!, \label{ineq:estimateg_i}
	\end{align}
	where the second inequality applies Assumption \ref{A1} and the last equality is a consequence of the claim $g_i(0,0) \neq 0$. Note that $D$ is linear in $\norm{u}_U$ and $C$ is linear in $\norm{x}_X$. Therefore, by \eqref{ineq:estimateofxinu}, $L_{g_i}^1$ and $L_{g_i}^2$ are weakly growing functions in $\norm{u}_U$. It can be seen that $\tilde{\alpha}_3(s) := L_{g_i}^1\!\para{\kappa^{-1}(s),s} \kappa(s)+ L_{g_i}^2\!\para{\kappa(s),s} s$ belongs to class $\mathcal{K}_\infty$. By defining the $\mathcal{K}_\infty$-function $\alpha_3 := \alpha_2\circ \tilde{\alpha}_3$ we conclude
	\begin{align*}
		V(t_i,g_i(x,u)) \leq \alpha_2\!\para{\norm{g_i(x,u)}_X} \leq \alpha_3\!\para{\norm{u}_U}.
	\end{align*}
	We used \eqref{ineq:LyapunovDefiniteness} in the first inequality and \eqref{ineq:estimateg_i} in the second one.	So, $V$ is an ISS-Lyapunov function for system \eqref{eq:ImpulsiveSystem}.
\end{pf}

We now state the following theorem, which summarizes the main results. Note, that the proof of the theorem also provides a formal proof of Theorem \ref{thm:inverseLyapunov}.

\begin{theorem}\label{thm:equivLyapunovStability}
	Let Assumption \ref{A1} hold. Then the following statements are equivalent:
	\begin{enumerate}[(i)]
		\item System \eqref{eq:ImpulsiveSystem} is ISS. \label{thm:mainstatement_1}
		\item System \eqref{eq:ImpulsiveSystem} is WURS. \label{thm:mainstatement_2}
		\item There exists an ISS-Lyapunov function for system \eqref{eq:ImpulsiveSystem}, which is Lipschitz continuous on bounded subsets of $X$ and locally Lipschitz continuous on $I \setminus S$ such that it is right continuous, and the left limit exists. \label{thm:mainstatement_3}
	\end{enumerate}
\end{theorem}

\begin{pf}
	By Theorem \ref{thm:Lyapunov}, Statement \ref{thm:mainstatement_3} implies Statement \ref{thm:mainstatement_1}.
	Lemma \ref{lem:WURS} implies that for every system that fulfills Statement \ref{thm:mainstatement_1}, Statement \ref{thm:mainstatement_2} also holds true.
	
	It remains to show the implication from Statement \ref{thm:mainstatement_2} to Statement \ref{thm:mainstatement_3}: We assume system \eqref{eq:ImpulsiveSystem} to be WURS. Then feedback system \eqref{eq:feedbackImpulsiveSystem} is UGAS for all $d \in D$ with  $\eta$ and $\psi$ as given in Definition \ref{def:WURS}. Proposition \ref{prop:Lipschitzcontinuity} then gives us that every solution of system \eqref{eq:feedbackImpulsiveSystem} is Lipschitz continuous with respect to initial values in bounded subsets of $X$, and locally Lipschitz continuous on the intervals $[t_i,t_{i + 1})$, $i \in \N_0$. Theorem \ref{thm:existenceOfLyapunovFunction} ensures that there exists a Lyapunov function $V: I \times X \to \R^+_0$ for  feedback system \eqref{eq:feedbackImpulsiveSystem}, which is Lipschitz continuous on bounded balls in space and locally Lipschitz continuous on the intervals $[t_i,t_{i + 1})$, $i \in \N_0$. From Lemma \ref{lem:WURStoISS} follows the existence of an ISS-Lyapunov function for system \eqref{eq:ImpulsiveSystem} as stated in the theorem.
\end{pf}



==> chapters/09_example.tex <==
{\color{blue}
\section{Illustrative Example}\label{sec:example}
% In this section, we provide three examples to illustrate the usefulness of our result.

% \subsection{Example 1}
% We consider a linear system without inputs for which ISS cannot be concluded with the candidate ISS-Lyapunov function. The focus is set on explaining why the candidate ISS-Lyapunov function method does not work, and how the present paper resolves this issue by proposing a time-varying ISS-Lyapunov function.

% Let us investigate the two-dimensional system
% \begin{align}\label{eq:IDEexample}
% 	\begin{aligned}
% 		\dot{x}(t) &= Ax, \qquad &&t \in \R_0^+ \setminus S, \\
% 		x(t) &= Bx^-, \qquad &&t \in S, \\
% 		x(0) &= x_0,
% 	\end{aligned}
% \end{align}
% equipped with Euclidean norm $\norm{\ph}$, where 
% $
% 	A := 
% 	\begin{pmatrix}
% 		1	&0 \\
% 		0	&-1
% 	\end{pmatrix}
% 	$, $B := 
% 	\begin{pmatrix}
% 		\frac{1}{2}	&0 \\
% 		0	&\frac{3}{2}
% 	\end{pmatrix}
% $
% with $S = \braces{t_i}_{i \in \N}$, and $t_i = \frac{1}{2} i$ for $i \in \N$.
% As this system does not have inputs, we will show that it is asymptotically stable. In direction of the first unit vector, the system reduces to
% \begin{align}\label{eq:exampleSystem1}
% 	\begin{aligned}
% 		\dot{x}_1(t) &= x_1, \qquad &&t \in \R_0^+ \setminus S, \\
% 		x_1(t) &= \frac{1}{2} x_1^-(t), \qquad &&t \in S.
% 	\end{aligned}
% \end{align}
% Obviously, the flow is unstable and the jumps are stable. The solution of the system is given by
% \begin{align*}
% 	x_1(t) = \frac{1}{2^{\lfloor 2t \rfloor}}e^t x_0,
% \end{align*}
% where $\lfloor \ph \rfloor$ is the floor function, which returns the largest integer smaller than the argument. By analysis of the limit, one can  see that system \eqref{eq:exampleSystem1} is stable.

% Fig. \ref{fig:Componentplotsa} shows a plot of the trajectory of system \eqref{eq:IDEexample} with initial condition $x_0 = 
% \begin{psmallmatrix*}
%     1 \\ 0
% \end{psmallmatrix*}
% $. While the trajectory in the direction of the second unit vector always stays zero, we have unstable flows in the first component, which are stabilized by jumps.

% We investigate the system induced by the second unit vector
% \begin{align}\label{eq:exampleSystem2}
% 	\begin{aligned}
% 		\dot{x}_2(t) &= -x_2, \qquad &&t \in \R_0^+ \setminus S, \\
% 		x_2(t) &= \frac{3}{2} x_2^-, \qquad &&t \in S.
% 	\end{aligned}
% \end{align}
% The solution here is given by
% \begin{align*}
% 	x_2(t) = \para{\frac{3}{2}}^{\lfloor 2t \rfloor}e^{-t} x_0.
% \end{align*}
% Therefore, the jumps are unstable, but the flow stabilizes the entire system.

% Fig. \ref{fig:Componentplotsb} shows a plot of the evolution of system \eqref{eq:IDEexample} with initial condition $x_0 = 
% \begin{psmallmatrix*}
%     0 \\ 1
% \end{psmallmatrix*}
% $. In the direction of the first unit vector, the system remains zero, but in the direction of the second unit vector, we can  see that the flow stabilizes the unstable jumps.

% \begin{figure}[tb]
%     \begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			\begin{axis}[
% 			        legend style={at={(1,1.2)},
% 						anchor=north east,legend columns=1},
% 					axis x line=bottom,
% 					axis y line=center,
% 					xlabel style={below},
% 					ylabel style={above},
% 					xmin=0,
% 					xmax=5.1,
% 					ymin=0,
% 					ymax=1.85,
% 					xlabel=time $t$,
% 					ylabel={state $(x_1,x_2)$},
% 					width=1\textwidth
% 				]
% 				\addplot[color=tuklblue,thick,unbounded coords=jump]table[x=t,y=x_1] {images/Ex1_UFSJ.txt};
% 				\addplot[color=tuklred,thick]table[x=t,y=x_2] {images/Ex1_UFSJ.txt};
%                 \addplot[color=tuklblue,thick,dotted,unbounded coords=discard]table[x=t,y=x_1] {images/Ex1_UFSJ.txt};
% 				\legend{$x_1$,$x_2$}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\caption{Plot of system \eqref{eq:IDEexample} with unstable flow and stable jumps for initial condition $x_0 = 
% 		\begin{psmallmatrix*}
% 		    1 \\ 0
% 		\end{psmallmatrix*}
% 		$.\label{fig:Componentplotsa}}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			%\pgfplotsset{every axis legend/.append style={at={(0.420,0.86)},anchor=south}}
% 			\begin{axis}[legend columns={1},
% 					legend style={at={(1,1.2)},
% 						anchor=north east,legend columns=1},
% 					axis x line=bottom,
% 					axis on top=false,
% 					axis y line=center,
% 					xlabel style={below},
% 					ylabel style={above},
% 					xmin=0,
% 					xmax=5.1,
% 					ymin=0,
% 					ymax=1.85,
% 					xlabel=time $t$,
% 					ylabel={state $(x_1,x_2)$},
% 					%xticklabel style={yshift=0mm},
% 					width=1\textwidth
% 					%,ylabel style={yshift=-1mm}
% 					%,xlabel style={yshift=1mm}
% 				]
% 				%\addplot[color=tuklblue,very thick] coordinates {(0,0) (3, 0)};
% 				\addplot[color=tuklblue, thick]table[x=t,y=x_1] {images/Ex1_SFUJ.txt};
% 				\addplot[color=tuklred,thick,unbounded coords=jump]table[x=t,y=x_2] {images/Ex1_SFUJ.txt};
% 				\addplot[color=tuklred,thick,dotted,unbounded coords=discard]table[x=t,y=x_2] {images/Ex1_SFUJ.txt};
% 				\legend{$x_1$,$x_2$}
% 			\end{axis}
% 		\end{tikzpicture}
% 		\caption{Plot of system \eqref{eq:IDEexample} with stable flow and unstable jumps for initial condition $x_0 = 
% 		\begin{psmallmatrix*}
% 		    0 \\ 1
% 		\end{psmallmatrix*}
% 		$.\label{fig:Componentplotsb}}
% 	\end{subfigure}
% 	\caption{Plots of two trajectories of system \eqref{eq:IDEexample}.\label{fig:Componentplots}}
% \end{figure}

% %\begin{figure}
% %	\begin{tikzpicture}
% %		%\pgfplotsset{every axis legend/.append style={at={(0.420,0.86)},anchor=south}}
% %		\begin{axis}[legend columns={1},
% %				%legend style={at={(0.84,0.98)},anchor=north east},
% %				axis x line=center,
% %				axis y line=center,
% %				xlabel style={below right},
% %				ylabel style={above},
% %				xmin=0,
% %				xmax=3.1,
% %				ymin=0,
% %				ymax=1.8,
% %				xlabel=time $t$,
% %				ylabel={state $(x_1,x_2)$},
% %				%xticklabel style={yshift=0mm},
% %				width=0.54\textwidth
% %				%,ylabel style={yshift=-1mm}
% %				%,xlabel style={yshift=1mm}
% %			]
% %			\addplot[color=tuklblue,very thick]table[x=t,y=x_1] {images/IDE_uflow_sjump.txt};
% %			\addplot[color=tuklred,very thick]table[x=t,y=x_2] {images/IDE_uflow_sjump.txt};
% %			%\addplot[color=tuklblue,dashed,thick]table[x=x,y=beta1] {data/birthhh.txt};
% %			%\addplot[color=tuklred,thick]table[x=x,y=mu0] {data/birthh.txt};
% %			%\addplot[color=tuklred,dashed,thick]table[x=x,y=mu1] {data/birthhh.txt};
% %			\legend{$x_1$,$x_2$}
% %		\end{axis}
% %	\end{tikzpicture}
% %\end{figure}

% The approach via candidate ISS-Lyapunov functions cannot  prove ISS of the system defined in \eqref{eq:IDEexample} because it has unstable flow in one direction and unstable jumps in the other one. Results like \cite{Dashkovskiy2013}, \cite{Hespanha2008},  and also the authors' own recent paper \cite{Bachmann2020} were only able to deal with one of the subsystems \eqref{eq:exampleSystem1} or \eqref{eq:exampleSystem2} because they only consider the upper bound of the flow and jump dynamics, respectively. So, an ISS statement is not possible with candidate ISS-Lyapunov functions.

% With the paper at hand, we fill this gap and provide an ISS-Lyapunov function.
% In the present case, an ISS-Lyapunov function is given by
% \begin{align}\label{eq:ex1Lyapfunction}
% 	V(t,x) := x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} x.
% \end{align}
% $V$ is indeed an ISS-Lyapunov function as we show by checking the requirements of Definition \ref{def:LyapunovFunction}.
% \begin{enumerate}
% 	\item $V(t,x) = \para{\frac{1}{4}}^{2t - \lfloor 2t \rfloor}x_1^2 + \para{\frac{9}{4}}^{2t - \lfloor 2t \rfloor}x_2^2$, and therefore
% 	\begin{align*}
% 		\frac{1}{4}\norm{x}^2 \leq V(t,x) \leq \frac{9}{4} \norm{x}^2.
% 	\end{align*}
% 	\item As system \eqref{eq:IDEexample} does not have inputs, the inequalities \eqref{ineq:LyapunovFlow} and \eqref{ineq:LyapunovJump} must be satisfied independently of $u$.
% 	\begin{align*}
% 		&\frac{\diff}{\diff t} V(t,x) \\
% 		&= 4 x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} \ln(B) x \\
% 		&\quad+ 2 x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} Ax \\
% 		&= x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} \brackets{4 \ln(B) + 2A} x.
% 	\end{align*}
% 	The term
% 	\begin{align*}
% 		&4 \ln(B) + 2A \\
% 		&=
% 		\begin{pmatrix}
% 			-4 \ln(2) + 2	&0 \\
% 			0				&4 \ln(3) - 4 \ln(2) - 2
% 		\end{pmatrix} \\
% 		&\approx
% 		\begin{pmatrix}
% 			-0.773	&0 \\
% 			0				&-0.378
% 		\end{pmatrix},
% 	\end{align*}
% 	can be bounded from above by $- 0.3 I$. As a consequence, we have
% 	\begin{align*}
% 		&\frac{\diff}{\diff t} V(t,x) \\
% 		&= x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} \brackets{4 \ln(B) + 2A} x \\
% 		&\leq -0.3 x^T \para{B^{2t - \lfloor 2t \rfloor}}^T B^{2t - \lfloor 2t \rfloor} x \\
% 		&= -0.3 V(t,x)
% 	\end{align*}
% 	for all initial conditions $x_0 \in X$ and all $t \in I \setminus S$. Moreover, $V$ fulfills
% 	\begin{align}\label{eq:ExampleLyapunovInequalityJump}
% 		V\!\para{t_i, Bx} &= x^TB^T \para{B^0}^T B^0 Bx \nonumber\\
% 		&= x^T \para{B^1}^T B^1 x = V\!\para{t_i^-, x},
% 	\end{align}
% 	which is exactly \eqref{ineq:LyapunovJump}.
% 	\item Inequality \eqref{def:LyapFuncCondition3} is fulfilled by \eqref{eq:ExampleLyapunovInequalityJump} as we set
% 	\begin{align*}
% 		V(t_i,Bx) = V\!\para{t_i^-, x}  < \chi\!\para{\norm{u}_\infty}
% 	\end{align*}
% 	for all $\mathcal{K}_\infty$-functions $\chi$. We can then choose $\alpha_3 := \chi$.
% \end{enumerate}
% Thus, by applying Theorem \ref{thm:equivLyapunovStability}, we can conclude that system \eqref{eq:IDEexample} is asymptotically stable.

% It is interesting to observe the Lyapunov function's behavior, which is sketched in Fig. \ref{fig:Lyapfunction}. The function is periodic with jumps at $t = 0.5 \N$. In the interval $[0.5 i-0.5, 0.5i)$, $i \in \N$, the Lyapunov function is continuous. It can be seen that the Lyapunov function funnel is rising in the $x_2$-direction during the flow. At the same time, it is opening in the $x_1$-direction. Therefore, the trajectories in the $x_1$-direction move away from the origin during the flow. So, the Lyapunov value has to fall faster than each of the trajectories diverges.
% At the moment of jump, the Lyapunov function bounces back to the initial state because the trajectories move much closer to the origin than in the initial condition.
% For the $x_2$-direction, it is vice versa. At the jump, the trajectories increase their distance to the origin, so the Lyapunov function has to catch the trajectory, such that the Lyapunov value of the trajectory is not increasing.

% \begin{figure}[tb]
% 	\begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			\begin{axis}[
% 					title={$t = 0$},
% 					xlabel={$x_1$},
% 					ylabel={$x_2$},
% 					zlabel={$V(0,x)$},
% 					grid,
% 					xticklabels=\empty,
% 					yticklabels=\empty,
% 					zticklabels=\empty,
% 					x label style={yshift=+.6em},
% 					y label style={yshift=+.9em,xshift=-.4em},
% 					z label style={yshift=-.6em},
% 					shader=interp,
% 					colormap/blackwhite,
% 					zmin=0,
% 					zmax=11,
% 					width=1.15\textwidth,
% 					height=.9\textwidth
% 				]
% 				\addplot3[surf,mesh/rows=21,mesh/ordering=y varies,mesh/check=false] table{images/Ex1_LF1.txt};
% 			\end{axis}
% 		\end{tikzpicture}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			\begin{axis}[
% 					title={$t = 0.25$},
% 					xlabel={$x_1$},
% 					ylabel={$x_2$},
% 					zlabel={$V(0.25,x)$},
% 					grid,
% 					xticklabels=\empty,
% 					yticklabels=\empty,
% 					zticklabels=\empty,
% 					x label style={yshift=+.6em},
% 					y label style={yshift=+.9em,xshift=-.4em},
% 					z label style={yshift=-.6em},
% 					shader=interp,
% 					colormap/blackwhite,
% 					zmin=0,
% 					zmax=11,
% 					width=1.15\textwidth,
% 					height=.9\textwidth
% 				]
% 				\addplot3[surf,mesh/rows=21,mesh/ordering=y varies,mesh/check=false] table{images/Ex1_LF2.txt};
% 			\end{axis}
% 		\end{tikzpicture}
% 	\end{subfigure}
% 	\begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			\begin{axis}[
% 					title={$t = 0.5^-$},
% 					xlabel={$x_1$},
% 					ylabel={$x_2$},
% 					zlabel={$V^-(0.5,x)$},
% 					grid,
% 					xticklabels=\empty,
% 					yticklabels=\empty,
% 					zticklabels=\empty,
% 					x label style={yshift=+.6em},
% 					y label style={yshift=+.9em,xshift=-.4em},
% 					z label style={yshift=-.6em},
% 					shader=interp,
% 					colormap/blackwhite,
% 					zmin=0,
% 					zmax=11,
% 					width=1.15\textwidth,
% 					height=.9\textwidth
% 				]
% 				\addplot3[surf,mesh/rows=21,mesh/ordering=y varies,mesh/check=false] table{images/Ex1_LF3.txt};
% 			\end{axis}
% 		\end{tikzpicture}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}[c]{0.23\textwidth}
% 		\begin{tikzpicture}
% 			\begin{axis}[
% 					title={$t = 0.5$},
% 					xlabel={$x_1$},
% 					ylabel={$x_2$},
% 					zlabel={$V(0.5,x)$},
% 					grid,
% 					xticklabels=\empty,
% 					yticklabels=\empty,
% 					zticklabels=\empty,
% 					x label style={yshift=+.6em},
% 					y label style={yshift=+.9em,xshift=-.4em},
% 					z label style={yshift=-.6em},
% 					shader=interp,
% 					colormap/blackwhite,
% 					zmin=0,
% 					zmax=11,
% 					width=1.15\textwidth,
% 					height=.9\textwidth
% 				]
% 				\addplot3[surf,mesh/rows=21,mesh/ordering=y varies,mesh/check=false] table{images/Ex1_LF1.txt};
% 			\end{axis}
% 		\end{tikzpicture}
% 	\end{subfigure}
% 	\caption{Evolution of the Lyapunov function with time. \label{fig:Lyapfunction}}
% \end{figure}

% \subsection{Example 2}
% We extend the insights from the first example to a nonlinear system with input. ISS of this system is also not provable with the traditional approach of candidate ISS-Lyapunov functions as the system is strictly unstable in both components of the flow and  the direction of the first unit vector of the jumps. Only the jump direction of the second unit vector is stable.

% To this end, we consider the two-dimensional system in $\R^2$ equipped with Euclidean norm $\norm{\ph}$ and $u \in \R$,
% \begin{align}\label{eq:IDEexample2}
% 	\begin{aligned}
% 		\dot{x}(t) &= Ax, \qquad &&t \in \R_0^+ \setminus S, \\
% 		x(t) &= g\!\para{x^-(t),u}, \qquad &&t \in S, \\
% 		x(0) &= x_0,
% 	\end{aligned}
% \end{align}
% where 
% $
% 	A := 
% 	\begin{pmatrix}
% 		1	&1 \\
% 		-1	&1
% 	\end{pmatrix}
% 	$, $g\!\para{\begin{pmatrix}
%     x_1 \\
%     x_2
% \end{pmatrix},u} := 
% 	\begin{pmatrix}
% 		2 x_1 \\
% 		u \tanh(x_2)
% 	\end{pmatrix}
% $
% with $S = \braces{t_i}_{i \in \N}$, and $t_i = \frac{\pi}{2} i$ for $i \in \N$.

% We show that
% \begin{align*}
%     V(t,x) = e^{-4(t-t_n)} x^T R\!\para{t-t_n}D R^T\!\para{t-t_n}x,
% \end{align*}
% where $n = \max\!\braces{i \in \N\,\middle| \, t_i \leq t}$, is an ISS-Lyapunov function for system \eqref{eq:IDEexample2} with function $\chi(s) = 8 e ^{6 \pi} s^2$. Here, $R$ is the rotation matrix and $D$ is the diagonal matrix defined by
% \begin{align*}
%     R(t) = 
%     \begin{pmatrix}
%         \cos(t)     &\sin(t) \\
%         -\sin(t)    & \cos(t)
%     \end{pmatrix}
%     ,\quad D =
%     \begin{pmatrix}
%         \frac{1}{4} &0 \\
%         0           &2e^{2 \pi}
%     \end{pmatrix},
% \end{align*}
% respectively. We show the properties in Definition~\ref{def:LyapunovFunction}.
% \begin{enumerate}
%     \item Obviously,
%     \begin{align*}
%         \frac{1}{4}e^{-2\pi} \norm{x}^2 \leq V(t,x) \leq 2 e^{2\pi} \norm{x}^2
%     \end{align*}
%     holds for all $(t,x) \in \R^+_0 \times \R^2$.
%     \item The time-derivative of $V$ along the trajectories of the system \eqref{eq:IDEexample2} is given by
%     \begin{align*}
% 		&\frac{\diff}{\diff t} V(t,x) \\
% 		&= -4 e^{-4(t-t_n)}x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} x \\
% 		&\quad + 2 e^{-4(t-t_n)} x^T R\!\para{t-t_n} D \dot{R}^T\!\para{t-t_n} x \\
% 		&\quad + 2 e^{-4(t-t_n)} x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} A x \\
% 		&= -2 e^{-4(t-t_n)}x^T R\!\para{t-t_n} D R^T\!\para{t-t_n} x \\
% 		&= -2 V(t,x)
% 	\end{align*}
% 	for all $x \in \R^2$ and $t \in I \setminus S$ as the second last line follows from the fact that $R^T A = R^T - \dot{R}^T$. Since $2e^{2\pi}\norm{x}^2\geq V(t,x) \geq \chi\!\para{\norm{u}_\infty} = 8e^{6 \pi} \!\norm{u}_\infty^2$ holds, we obtain
% 	\begin{align*}
% 	    V\!\para{t_i,g(x,u)} &= e^0 g(x,u)^T R(0)DR^T(0)g(x,u) \\
% 	    &= x_1^2 + 2e^{2\pi}u^2\tanh^2(x_2) \\
% 	    &\leq e^{-2\pi} \para{2e^{2\pi}x_1^2 + \frac{1}{4}x_2^2} \\
% 	    &= e^{-4\cdot\frac{\pi}{2}}x^T R\!\para{\frac{\pi}{2}}DR^T\!\para{\frac{\pi}{2}}x \\
% 	    &= V(t_i^-,x)
% 	\end{align*}
% 	for each $i \in \N$ and all $x \in \R^2$.
% 	\item For $V(t,x) < \chi\!\para{\norm{u}_\infty} = 8e^{6 \pi} \norm{u}_\infty^2$, we have
% 	\begin{align*}
% 	    V\!\para{t_i,g(x,u)} &= x_1^2 + 2e^{2\pi} u^2\tanh^2(x_2) \\
% 	    &\leq 2e^{2\pi}\norm{x}^2 \cdot \max\!\braces{1, u^2} \\
% 	    &\leq 64e^{10\pi}\norm{u}_\infty^2 \cdot \max\!\braces{1, \norm{u}_\infty^2},
% 	\end{align*}
% 	as by property (1), $\norm{x}^2 \leq 4 e^{2\pi} V(t,x)$ holds.
% \end{enumerate}
% Therefore, $V$ is indeed an ISS-Lyapunov function. By Theorem \ref{thm:Lyapunov}, system \eqref{eq:IDEexample2} is ISS.

%\subsection{Example 3}

In order to illustrate the applicability of ISS-Lyapunov functions, we study an infinite-dimensional example, i.e.,
%Finally, in order to illustrate the applicability of our result to infinite-dimensional systems, we study an example with 
a PDE over the Banach space $\para{\lin^2\!\para{[-1,1]}, \norm{\ph}_2}$. Thereby, we consider the flow to be an inhomogeneous heat equation of the type $\dot{x} = a \tfrac{\partial^2}{\partial y^2} x + f(t,x,y)$. Its solution is parametrized by $x(t) = x(t,y)$ for $y \in [-1,1]$. 

We state the following problem
\begin{align}\label{eq:IDEexample3}
    \begin{aligned}
        \tfrac{\diff}{\diff t} x(t,y) 
        &= a \cdot\tfrac{\partial^2}{\partial y^2} x(t,y) + f(t,x,y), \quad &&t \in \R^+_0 \setminus S,\\
        x(t,y) 
        &= g\!\para{x^-(t,y),y,u}, \quad &&t \in S,
    \end{aligned}
\end{align}
where $x(t,-1) = x(t,1) = 0$ for all $t \in \R^+_0$ and $a > 0$ is the thermal diffusivity. We assume $\abs{f(t,x,y)} \leq \abs{x(t,y)}$ and $\abs{g\!\para{x^-(t,y),y,u}} \leq \sqrt{\abs{u}\norm{x}_2}$. The jump times are given by $S = \braces{t_i \in \R\,\middle|\,i \in \N}$, where $t_i = c i$ for some constant $c \in (0,\tfrac{1}{2}]$ and $u: \R \to \R$ is bounded.

We show this system is ISS by using the Lyapunov function
\begin{align*}
    V(t,x) &= \big\|e^{-h(t)}x(t,\ph)\big\|_2^2,
\end{align*}
where $h(t) := \frac{t-t_n}{\para{t_{n+1}-t_n}} - \frac{1}{2}$ for $t \in [t_n,t_{n+1})$, and the function $\chi(s) = 4 e^5 s^2$.

\begin{figure}
    \centering
    \begin{subfigure}[c]{0.45\textwidth}
        \begin{tikzpicture}
        	\begin{axis}[
                	%axis line style={shorten >=-1cm, shorten <=-20pt},
        	        axis lines*=left,
                    z axis line style={-stealth},
        			%title={$t = 0.5$},
        			xlabel={time $t$},
        			ylabel={space $y$},
        			zlabel={state $x(t,y)$},
        			%grid,
        			zmajorgrids=true,
        			%xticklabels=\empty,
        			%yticklabels=\empty,
        			%zticklabels=\empty,
        			x label style={yshift=+.6em},
        			y label style={yshift=+.9em,xshift=-.4em},
        			z label style={yshift=-.6em},
        			shader=interp,
        			%colormap/blackwhite,
        			zmin=0,
        			zmax=3,
        			width=1\textwidth,
        			height=0.7\textwidth,
        			x tick label style={
        			    /pgf/number format/.cd,
        			    scaled x ticks = false,
        			    fixed
        			},
        			z tick label style={
        			    yshift=+.4em
                    },
        		]
        % 		%Lyapunov value background fill
        % 		\addplot3[
        %         	fill=tuklblue!70,
        %         	fill opacity=0.75,
        %             draw=black,dotted,
        %             mark=none,
        %     	] table[, x = time, y expr = 1, z = value]{images/LyapExamp3-2.txt};
            	
        %     	% Lyapunov value
        %     	\addplot3[
        %         	black,
        %         	unbounded coords=jump,
        %     	] table[, x = time, y expr = 1, z = value]{images/LyapExamp3-2.txt};
            	
        %     	% dotted lines between jumps of Lyapunov values
        %     	\addplot3[
        %         	domain=0:0.2,
        %         	samples=3,
        %         	samples y=0,
        %         	tuklred,
        %         	thick,
        %         	unbounded coords=jump
        %      	] (x,1,1.28402);
            	
            	% 3D-plot of state evolution
            	\addplot3[surf,
            		shader=faceted interp,
            		%opacity=0.5,
            		mesh/rows=11,
            		mesh/ordering=y varies,
            		mesh/check=false,
            		unbounded coords=jump
        		] table{images/Ex3_states.txt};
        	\end{axis}
        \end{tikzpicture}
        \caption{Time evolution of the state  of system~\eqref{eq:IDEexample3}.}
    \end{subfigure}
    \begin{subfigure}[c]{0.45\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
			        %legend style={at={(1,1.2)},
					%	anchor=north east,legend columns=1},
					axis x line=center,
					axis y line=center,
					xlabel style={right},
					ylabel style={right},
					x tick label style={
					    /pgf/number format/.cd,
					    scaled x ticks = false,
					    fixed,
					    fixed zerofill,
					    precision=1},
					y tick label style={
                        /pgf/number format/.cd,
                        scaled y ticks = false,
                        fixed,
                        %fixed zerofill,
                        %precision=2
                    },
				 	xmin=0,
				    xmax=2.1,
				 	ymin=0,
					ymax=11,
					xlabel=time $t$,
					ylabel={Lyapunov value $V(t,x)$},
					width=.85\textwidth,
					height=0.5\textwidth,
					extra y tick labels={$\chi\!\para{\norm{u}_\infty}$},
					extra y ticks={5.94},
					extra y tick style = {
    					tuklred,
    					every tick/.append style={tuklred,thick},
    					tick label style={yshift={2mm}}
    				},
				]
    				
          		% Lyapunov dotted interconnections
        		\addplot[color=tuklblue,
        		very thick,
        		dotted,
        		unbounded coords=discard
        		] table{images/Ex3_LF.txt};
            	
            	% Lyapunov value
            	\addplot[color=tuklblue,
            	very thick,
            	unbounded coords=jump
            	] table{images/Ex3_LF.txt};
            	
            	% dotted lines between jumps of Lyapunov values
            	\addplot[
                	domain=0:2,
                	samples=2,
                	samples y=0,
                	tuklred,
                	thick,
                	unbounded coords=jump
             	] (x,5.94);
        	\end{axis}
        \end{tikzpicture}
        \caption{A plot of the Lyapunov function value. The red line illustrates the perturbation radius $\chi\!\para{\norm{u}_\infty} = 4e^5\norm{u}_\infty^2$.}
    \end{subfigure}
    \caption{Simulation of system \eqref{eq:IDEexample3} with $a = 0.1$, $f(t,x,u) = 2x$, $g(x,y,u) = \sqrt{\abs{u} \norm{x}}$, initial value $x(0,y) = 2(y^2-1)^2$ and input $u \equiv 0.1$. The jumps have periodicity $c = 0.5$. \label{fig:LyapfunctionExample3}}
\end{figure}

Indeed, $V$ is an ISS-Lyapunov function, as we show by following the conditions of Definition \ref{def:LyapunovFunction}.
\begin{enumerate}
    \item It can be easily seen that $\tfrac{1}{e} \norm{x}_2^2 \leq V(t,x) \leq e\norm{x}_2^2$ holds for all $t \in \R^+_0$, and all $x \in \lin^2\!\para{[-1,1]}$.
    \item The time-derivative of $V$ fulfills 
    \begin{align*}
        &\tfrac{\diff}{\diff t} V(t,x) 
        = \int_{-1}^{1} 2e^{-h(t)}x(t,y) \left(-\dot{h}(t)e^{-h(t)}x(t,y) \right. \\
        &\qquad\left.+ e^{-h(t)} \para{a x''(t,y) + f(t,x,y)}\right) \, \diff y\\
        &\leq \int_{-1}^{1} 2a e^{-2h(t)}x(t,y) x''(t,y) \, \diff y\\
        &= -2a e^{-2h(t)}\int_{-1}^{1} x'(t,y) x'(t,y) \, \diff y\\
        &= - 2a e^{-2h(t)}\norm{x'}_2^2
        \leq -\tfrac{a}{2} e^{-2h(t)}\norm{x}_2^2
        \leq - \tfrac{a}{2} V(t,x).
    \end{align*}
    In the second step, we applied $\dot{h}(t) = \frac{1}{\para{t_{n+1}-t_n}} \geq 1$. In the third step, we used Green's first identity. In the second last step, we used the fact $\norm{x}_2 \leq 2\norm{x'}_2$, which follows from Friedrichs's inequality.
    
    The jumps satisfy
    \begin{align*}
        &V\!\para{t_i,g\!\para{x(t_i,\ph), u}} 
        = \big\|e^{-h(t_i)} g\!\para{x(t_i,\ph), u}\big\|_2^2 \\*
        &= \big\|e^{1 - h^-(t_i)} g\!\para{x(t_i,\ph), u}\big\|_2^2
        = V^-\!\para{t_i,x(t_i,\ph)}
    \end{align*}
    because $\abs{g\!\para{x(t,y),u}} \leq  \sqrt{\abs{u}\norm{x}_2} \leq \tfrac{1}{\sqrt{2}e} \norm{x}_2$ as $e\norm{x}_2^2 \geq V(t,x) \geq \chi\!\para{\norm{u}_\infty} = 4 e^5\norm{u}_\infty^2$ holds.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item If $V(t,x) < \chi\!\para{\norm{u}_\infty}$, i.e., $\tfrac{1}{e} \norm{x}_2^2 \leq V(t,x) < \chi\!\para{\norm{u}_\infty} = 4e^5 \norm{u}_\infty^2$ holds, then follows
    \begin{align*}
        V\!\para{t_i,g\!\para{x(t_i,\ph), u}} 
        &= \big\|e^{-h(t_i)}g\!\para{x(t_i,\ph), u}\big\|_2^2 \\
        &\leq 4e^4 \norm{u}_\infty^2.
    \end{align*}
\end{enumerate}
Hence, we determined that $V$ is an ISS-Lyapunov function and by Theorem \ref{thm:Lyapunov}, system \eqref{eq:IDEexample3} is ISS.

Fig. \ref{fig:LyapfunctionExample3}a shows the time-evolution of the state of system \eqref{eq:IDEexample3}. %It is evident from the picture that the system state is falling until it reaches the perturbation radius $\chi\!\para{\norm{u}}$. 
Fig. \ref{fig:LyapfunctionExample3}b shows a plot of the Lyapunov function value, where the red line represents the perturbation radius $\chi\!\para{\norm{u}_\infty}$.
It is evident that the Lyapunov value of the system state is falling until it reaches the perturbation radius. After falling below, the Lyapunov value of the system state remains bounded.
}



==> chapters/13_example.tex <==
\section{Example}\label{sec:example}
\task{DRAFT:

\task{Define coercive operator}


We consider system \eqref{eq:ImpulsiveSystem} on a Hilbert space $X$ with
\begin{align*}
    f(t, x, u) &= Bu + \tilde f(x,u), \\
    g_i(x, u) &= Cx + Du + \tilde g(x, u),
\end{align*}
where $B, D \in L(U, X)$, $C \in L(X,X)$ and $\tilde f, \tilde g: X \times U \to X$ fulfill $\norm{\tilde f(x,u)}_X, \norm{\tilde g(x,u)}_X \in o\!\para{\norm{x}_X + \norm{u}_U}$. Here $o$ denotes the Landau symbol. The impulsive system then takes the form
\begin{align}\label{eq:exImpulsiveSystem}
    \begin{aligned}
        \dot{x}(t) &= Ax(t) + Bu(t) + \tilde f\!\para{t,x(t),u(t)}, \ &&t \in I\setminus S, \\
    x(t) &= Cx(t) + Du(t) + \tilde g\!\para{x^-(t),u^-(t)}, \ &&t \in S.
    \end{aligned}
\end{align}
If the continuous system
\begin{align*}
    \begin{aligned}
        \dot{x}(t) &= Ax(t) + Cu(t)
    \end{aligned}
\end{align*}
is ISS and if there exists a bounded coercive operator $P$ satisfying
\begin{align*}
    \sk{Ax}{Px} + \sk{Px}{Ax} = -\norm{x}_X \quad \forall x\in D(A),
\end{align*}
then a LISS-Lyapunov function of \eqref{eq:exImpulsiveSystem} is given by
$V(t,x) = \sk{Px}{x}$.
}
